GCformer: An Efficient Framework for Accurate and Scalable Long-Term Multivariate Time Series Forecasting

Transformer-based models have emerged as promising tools for time series forecasting. However, these model cannot make accurate prediction for long input time series. On the one hand, they failed to capture global dependencies within time series data. On the other hand, the long input sequence usually leads to large model size and high time complexity. To address these limitations, we present GCformer, which combines a structured global convolutional branch for processing long input sequences with a local Transformer-based branch for capturing short, recent signals. A cohesive framework for a global convolution kernel has been introduced, utilizing three distinct parameterization methods. The selected structured convolutional kernel in the global branch has been specifically crafted with sublinear complexity, thereby allowing for the efficient and effective processing of lengthy and noisy input signals. Empirical studies on six benchmark datasets demonstrate that GCformer outperforms state-of-the-art methods, reducing MSE error in multivariate time series benchmarks by 4.38% and model parameters by 61.92%. In particular, the global convolutional branch can serve as a plug-in block to enhance the performance of other models, with an average improvement of 31.93\%, including various recently published Transformer-based models. Our code is publicly available at https://github.com/zyj-111/GCformer.

==> tables/full_bench_multi.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{multivariate long-term series forecasting results on six datasets with various input length and prediction length $O \in \{96,192,336,720\}$ (For ILI dataset, we set prediction length $O \in \{24,36,48,60\}$). A lower MSE indicates better performance. All experiments are repeated 5 times.}\vspace{-1mm}
\scalebox{0.60}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
                        & 192 & \textbf{0.222} & \textbf{0.296} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
                        & 336 & \textbf{0.277} & \textbf{0.333} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
                        & 720 & \textbf{0.371} & \textbf{0.389} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} &96  &\textbf{0.154}  &\textbf{0.267}  &0.183 &0.297 &0.201  &0.317 &0.304 &0.405 &0.274  &0.368  &0.258  &0.357  &0.312  &0.402    \\
                        & 192 &\textbf{0.164} & \textbf{0.258} & 0.195 &0.308 &0.222  &0.334 &0.313 &0.413 &0.296 &0.386  &0.266 &0.368  &0.348  &0.433    \\
                        & 336 & \textbf{0.188} & \textbf{0.283} &0.212 &0.313 &0.231 &0.338 &0.290 &0.381 &0.300  &0.394  &0.280 &0.380  &0.350  & 0.433    \\
                        & 720 & 0.236 & \textbf{0.332} &\textbf{0.231} &0.343 &0.254  &0.361 &0.262 &0.344 &0.373  &0.439 &0.283  &0.376  &0.340  &0.420     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} &96  & \textbf{0.086} & \textbf{0.204} &0.139 &0.276 &0.197  &0.323 &1.292 &0.849 &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
                        & 192 & \textbf{0.188} & \textbf{0.292} &0.256 &0.369 &0.300  &0.369 &1.631 &0.968 &1.204   &0.895 &1.040  &0.851  &1.188  & 0.906   \\
                        & 336 & \textbf{0.356} & \textbf{0.433} &0.426 &0.464 &0.509  &0.524 &2.225 &1.145 &1.672  &1.036  &1.659  &1.081  &1.357  &0.976     \\
                        & 720 & \textbf{0.727} & \textbf{0.669} &1.090 &0.800 &1.447  &0.941 &2.521 &1.245 &2.478  &1.310  &1.941  &1.127  &1.510  &1.016     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} &96  &\textbf{0.416}& \textbf{0.294} &0.562 &0.349 &0.613  &0.388 &0.824 &0.514 &0.719  &0.391  &0.684  &0.384  &0.732  &0.423    \\
                        & 192 & \textbf{0.408} & \textbf{0.288} &0.562 &0.346 &0.616&0.382 &1.106 &0.672 &0.696 &0.379  &0.685  &0.390  &0.733  &0.420    \\
                        & 336 & \textbf{0.425} & \textbf{0.298} &0.570 &0.323 &0.622  &0.337 &1.084 &0.627 &0.777  &0.420  &0.733  &0.408  &0.742  &0.420     \\
                        & 720 & \textbf{0.520} &\textbf{0.353} &0.596 &0.368 &0.660  &0.408 &1.536 &0.845 &0.864  &0.472  &0.717  &0.396  &0.755  &0.423     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}} & 96 & \textbf{0.199} & \textbf{0.262} &0.217  &0.296  &0.266  &0.336 &0.406 &0.444 &0.300  &0.384  &0.458  &0.490  &0.689  &0.596    \\
                        & 192 & \textbf{0.228} & \textbf{0.288} &0.276  &0.336  &0.307  &0.367 &0.525 &0.527 &0.598  &0.544  &0.658  &0.589  &0.752  &0.638    \\
                        & 336 &\textbf{0.267} &\textbf{0.323} & 0.339  &0.380  &0.359  &0.395 &0.531 &0.539 &0.578  &0.523  &0.797  &0.652  &0.639  &0.596    \\
                        & 720 &\textbf{0.319} & \textbf{0.361} &0.403  &0.428 &0.578 &0.578 &0.419  &0.428  &1.059  &0.741  &0.869  &0.675  &1.130  &0.792    \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} & 24 & \textbf{1.970} & \textbf{0.875} &2.203  &0.963  &3.483 &1.287 &4.631 &1.484 &5.764  &1.677  &4.480  &1.444  &4.400 &1.382    \\
                        & 36 & \textbf{1.982} & \textbf{0.859} &2.272  &0.976  &3.103  &1.148 &4.123 &1.348 &4.755  &1.467  &4.799  &1.467  &4.783  &1.448    \\
                        & 48 & \textbf{1.868} & \textbf{0.896} &2.209  &0.981  &2.669  &1.085 &4.066 &1.36 &4.763  &1.469  &4.800  &1.468  &4.832  &1.465    \\
                        & 60 & \textbf{2.057} & \textbf{0.929} &2.545  &1.061  &2.770  &1.125 &4.278 &1.41 &5.264  &1.564  &5.278  &1.560  &4.882  &1.483    \\
\bottomrule
\end{tabular}
\label{tab:multi-benchmarks}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/full_bench_uni.tex <==
\begin{table*}[h]
% \begin{adjustwidth}{-1.5in}{-1in}
\centering
%\begin{small}
\caption{Univariate long-term forecasting results on six datasets with various input length and prediction horizon $O \in \{96,192,336,720\}$. A lower MSE indicates better performance. All experiments are repeated 5 times.}
\vskip 0.05in
\scalebox{0.60}{
\begin{tabular}{c|c|cccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 & 0.065 &\textbf{0.189}  &\textbf{0.063} &0.189 & 0.065 & 0.189 &0.153 &0.318 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 & \textbf{0.094} & \textbf{0.233} &0.102 &0.245 & 0.118 & 0.256 &0.183 &0.350 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 & \textbf{0.124} & \textbf{0.274} &0.130 &0.279 & 0.154 & 0.305 &0.204 & 0.367 &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 & \textbf{0.173} & \textbf{0.323} &0.178 &0.325 & 0.182 &0.335 &0.482 &0.567  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
& 96  & \textbf{0.154} & \textbf{0.247} &0.253 &0.370  &0.341 &0.438 &0.351 &0.452 & 0.484& 0.538 &0.288& 0.393& 0.274 & 0.379   \\
& 192 & \textbf{0.166} & \textbf{0.258} &0.282 &0.386 &0.345 &0.428 &0.373 &0.455 & 0.557& 0.558 &0.432 & 0.483 & 0.304 &0.402   \\
& 336 & \textbf{0.188} & \textbf{0.283} &0.346 &0.431 &0.406 &0.470 &0.408 &0.477 & 0.636& 0.613 &0.430 &0.483 & 0.370 &0.448  \\
& 720 & \textbf{0.249} & \textbf{0.341} &0.422 &0.484 &0.565 &0.581 &0.472 &0.517 & 0.819& 0.682 &0.491 &0.531 & 0.460 &0.511   \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
&96  & \textbf{0.110} & \textbf{0.259} &0.131 &0.284 & 0.241 & 0.387 &0.344 &0.482  & 0.591  &0.615  &0.237 &0.377  &0.298  &0.444    \\
& 192 & \textbf{0.207} & \textbf{0.352} &0.277 &0.420 &0.300  &0.369 &0.362 &0.494  &1.183   &0.912 &0.738  &0.619  &0.777  & 0.719   \\
& 336 & \textbf{0.327} & \textbf{0.461} &0.426 &0.511 &0.509  &0.524 &0.499 &0.594  &1.367  &0.984  &2.018  &1.070  &1.832  &1.128     \\
& 720 & \textbf{0.811} & \textbf{0.708} &1.162 &0.832 &1.260  &0.867 &0.552 & 0.614 &1.872  &1.072  &2.405  &1.175  &1.203  &0.956     \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
&96  & \textbf{0.144} & \textbf{0.215} &0.170 &0.263  &0.246 &0.346 &0.194 &0.290 & 0.257 & 0.353 &0.226 &0.317 &  0.313 & 0.383\\
& 192 & \textbf{0.120} & \textbf{0.199} &0.173 &0.265 &0.266 &0.370 &0.172 &0.272 & 0.299 & 0.376 &0.314 &0.408 & 0.386 & 0.453\\
& 336 & \textbf{0.128} & \textbf{0.212} &0.178 &0.266 &0.263 &0.371 &0.178 &0.278 & 0.312 & 0.387 &0.387 &0.453 & 0.423 & 0.468\\
& 720 & \textbf{0.153} & \textbf{0.252} &0.187 &0.286 &0.269 &0.372 &0.263 &0.386 & 0.366 & 0.436 &0.491 &0.437 & 0.378 & 0.433\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}}
& 96  & \textbf{0.0012} & \textbf{0.026} & 0.0035 & 0.046 & 0.011 &0.081 &0.0061 &0.065 & 0.0038 & 0.044 & 0.0046 &0.052 & 0.012 & 0.087 \\
& 192 & \textbf{0.0014}& \textbf{0.029}&0.0054 &0.059 &0.0075 &0.067 &0.0067 &0.067 & 0.0023 & 0.040 &0.0056 & 0.060 & 0.0098 & 0.079  \\
& 336 & \textbf{0.0015} & \textbf{0.030} &0.0041 &0.050 &0.0063 &0.062 &0.0025 &0.0381 & 0.0041 & 0.049 &0.0060 &0.054& 0.0050 & 0.059 \\
& 720 & \textbf{0.0022} & \textbf{0.037} &0.015 &0.091 &0.0085 &0.070 &0.0074 &0.0736 & 0.0031 & 0.042 &0.0071 &0.063& 0.0041 & 0.049 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
& 24 & \textbf{0.629} & \textbf{0.538} &0.693 &0.629 &0.948 &0.732 &0.866 &0.584 & 5.282 &2.050 &3.607 & 1.662 & 3.838 & 1.720  \\
& 36 & \textbf{0.444} & \textbf{0.481} &0.554 &0.604 &0.634 &0.650 &0.622 &0.532 & 4.554 &1.916 &2.407 & 1.363 & 2.934 & 1.520 \\
& 48 & \textbf{0.557} & \textbf{0.584} &0.699 &0.696 &0.791 &0.752 &0.813 &0.679 & 4.273 &1.846 &3.106 & 1.575 & 3.754 & 1.749\\
& 60 & \textbf{0.641} & \textbf{0.644} &0.828 &0.770 &0.874 &0.797 &0.931 &0.747 & 5.214 &2.057 &3.698 & 1.733 & 4.162 & 1.847\\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-large}
\vskip -0.10in
% \end{adjustwidth}
%\end{small}tab:multi-benchmarks
\end{table*}


==> tables/ks_test_small.tex <==

\begin{table}[h]
%\setlength{\uppercaptionskip}{0.pt}
%\setlength{\belowcaptionskip}{-0.pt}
%\vskip 0.15in
\centering
% \setlength{\belowcaptionskip}{2pt} 
\caption{P-values of Kolmogrov-Smirnov test of different Transformer models for long-term forecasting output on ETTm1 and ETTm2 dataset. Larger value indicates the hypothesis (the input sequence and forecasting output come from the same distribution) is less likely to be rejected. The largest results are highlighted.}
\begin{small}
% \begin{sc}
\vskip 0.05in
\scalebox{0.80}{
\begin{tabular}{c|c|cccccc}
\toprule
\multicolumn{2}{c|}{Methods}&Transformer&Informer&Autoformer&FEDformer&FiLM&True\\ %&\multicolumn{2}{c|}{Fedformer-f }\\%&\multicolumn{2}{c|}{}&\\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm1}} 
& 96 & 0.0090 & 0.0055&0.020 & \textbf{0.048} & 0.016& {0.023} \\
& 192 & 0.0052 & 0.0029&0.015 & \textbf{0.028} & 0.0123& {0.013} \\
& 336 & 0.0022 & 0.0019&0.012 & \textbf{0.015} & 0.0046& {0.010} \\
% & 720 & 0.0023 & 0.0016 & \textbf{0.014} & \textbf{0.0036} \\
& 720 & 0.0023 & 0.0016&0.008 & \textbf{0.014} & 0.0024& {0.004} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
% & 48 & 0.454 & & 0.366 & & 0.476 & & 0.356 \\
& 96 & 0.0012 & 0.0008& \textbf{0.079} &{0.071} & 0.022 & {0.087} \\%& \textbf{0.379} & \textbf{0.419}\\
& 192 & 0.0011 & 0.0006& \textbf{0.047} &{0.045}  &0.020 & {0.060} \\%& \textbf{0.426} & \textbf{0.441}\\
% & 288 & 0.634 & & 0.430 & & 0.571 & & 0.379 \\
& 336 & 0.0005 & 0.00009& 0.027 &\textbf{0.028} &0.012 & {0.042} \\%& \textbf{0.445} & \textbf{0.459}\\
% & 672 & 0.606 & & 0.528 & & 0.544 & & 0.501\\
& 720 & 0.0008& 0.0002& \textbf{0.023} & {0.021} &0.0081 & {0.023} \\
% \multicolumn{2}{c|}{Count}& 0 & 0 & 3 & 5 & 7& NA \\
%& \textbf{0.543} & \textbf{0.490}\\
%& -96 & 0.0012 & 0.0009 & 0.0001 & 0.0037 & \textbf{0.039} & \textbf{0.012} \\
\bottomrule
\end{tabular}
}
\label{tab:KStest_small}
% \end{sc}
\end{small}
%\end{center}
\vskip -0.1in
\end{table}




==> tables/tab_LPU_boosting.tex <==
%\resizebox{!}{\.5\paperheight}{
\vskip -0.1in
% \begin{wraptable}

% \begin{wraptable}[12]{r}{0.7\textwidth}
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Boosting effect of LPU layer for common deep learning backbones: MLP, LSTM, CNN and Attention.`+` indicates degraded performance.}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
%\begin{tabular}{c|c|cccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEL}&\multicolumn{2}{c|}{MLP}&\multicolumn{2}{c|}{LSTM}&\multicolumn{2}{c|}{lagged-LSTM}&\multicolumn{2}{c|}{CNN}&\multicolumn{2}{c}{Attention}\\
\midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\multicolumn{2}{c|}{Compare} & LPU  & Linear& LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030}  & +38\%   & 0.034  & +8.0\%  & 0.049 & +73\% & 0.093 & -21\% & 0.116   & -50\%   & 0.243  & -81\% \\
& 192  &\textbf{0.047} & +9.5\% & 0.049  & +30\%  & 0.174 & +32\% & 0.331 & -48\% & 0.101   & +20\%    & 0.387  & -86\% \\
& 336 & \textbf{0.063} & +5.8\% & 0.061  & +64\%  & 0.119 & +84\% & 0.214 & -19\% & 0.122   & +25\%    & 1.652  & +12\% \\
& 720 &\textbf{0.081} & +1.4\%  & 0.082  & +62\%  & 0.184 & +32\% & 0.303 & -6.5\%  & 0.108   & +13\%    & 4.782  & -61\% \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
% &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

&96  &\textbf{0.213}  & +136\%  & 0.431  & +121\%   & 0.291 & +55.6\% & 0.739 & -33\% & 0.310  & +43\%  & 0.805 & +23\% \\%&--& --
& 192 &\textbf{0.268} & +32\%   & 0.291 & +239\%   & 0.353  & +17\% & 0.535 & +15\% & 0.380  & +12\%  & 0.938 & +14\% \\%&--& --  \\
& 336 & \textbf{0.307}& +0.1\%  & 0.296 & +235\%   & 0.436  & -6.7\% & 0.517 & +23\% & 0.359  & +29\% & 2.043 & -54\% & \\%&--& -- \\
& 720 & \textbf{0.321}& +37\%   & 0.339 & +196\%   & 0.636  & -11\% & 0.492 & +28\% & 0.424  & +18\%  & 9.115 & +298\% \\ %&--& --  \\
 
\bottomrule
\end{tabular}
\label{tab:boosting}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
% \end{wraptable}
%}

==> tables/tab_LPU_boosting_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\vskip -0.1in
% \begin{wraptable}

%\begin{wraptable}[12]{r}{0.7\textwidth}
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{(Full Benchmark) Boosting effect of LPU layer for common deep learning backbones: MLP, LSTM, CNN and Attention.`+` indicates degraded performance.}\vspace{-1mm}
\scalebox{0.80}{
\begin{tabular}{c|c|cccccccccccccccccc}
%\begin{tabular}{c|c|cccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEL}&\multicolumn{2}{c|}{MLP}&\multicolumn{2}{c|}{LSTM}&\multicolumn{2}{c|}{lagged-LSTM}&\multicolumn{2}{c|}{CNN}&\multicolumn{2}{c}{Attention}\\
\midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\multicolumn{2}{c|}{Compare} & LPU  & Linear& LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear & LPU  & Linear\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030}  & +38\%   & 0.034  & +8.0\%  & 0.049 & +73\% & 0.093 & -21\% & 0.116   & -50\%   & 0.243  & -81\% \\
& 192  &\textbf{0.047} & +9.5\% & 0.049  & +30\%  & 0.174 & +32\% & 0.331 & -48\% & 0.101   & +20\%    & 0.387  & -86\% \\
& 336 & 0.063 & +5.8\% & \textbf{0.061}  & +64\%  & 0.119 & +84\% & 0.214 & -19\% & 0.122   & +25\%    & 1.652  & +12\% \\
& 720 &\textbf{0.081} & +1.4\%  & 0.082  & +62\%  & 0.184 & +32\% & 0.303 & -6.5\%  & 0.108   & +13\%    & 4.782  & -61\% \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 

&96  &\textbf{0.213}  & +136\%  & 0.431  & +121\%   & 0.291 & +56\% & 0.739 & -33\% & 0.310  & +43\%  & 0.805 & +23\% \\%&--& --
& 192 &\textbf{0.268} & +32\%   & 0.291 & +239\%   & 0.353  & +17\% & 0.535 & +15\% & 0.380  & +12\%  & 0.938 & +14\% \\%&--& --  \\
& 336 & 0.307& +0.1\%  & \textbf{0.296} & +235\%   & 0.436  & -6.7\% & 0.517 & +23\% & 0.359  & +29\% & 2.043 & -54\% & \\%&--& -- \\
& 720 & \textbf{0.321}& +37\%   & 0.339 & +196\%   & 0.636  & -11\% & 0.492 & +28\% & 0.424  & +18\%  & 9.115 & +298\% \\ %&--& --  \\
               
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
& 96  & 0.130 & +7.5\% & \textbf{0.110} & -18\% & 0.224 & +6.0\% & 0.521 & -58\% & 0.244 & -18\% & 0.338 & +872\% \\
& 192 & \textbf{0.205} & +39\% & 0.257 & -36\% & 0.787 & -35\% & 1.742 & -66\% & 0.630 & +2.1\% & 0.930 & +278\% \\
& 336 & 0.467 & +9.2\% & \textbf{0.461} & -33\% & 0.964 & +24\% & 2.281 & -38\% & 3.231 & -85\% & 1.067 & +69\%\\
& 720 & \textbf{1.003} & +26\% & 1.981 & -61\% & 2.703 & -29\% & 1.457 & +34\% & 5.531 & +9.7\% & 0.631 & +1831\% \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
&96  &\textbf{0.312} & +18\% & 0.376 & +277\% & 0.215 & +1.2\% & 0.216 & +10\% & 0.543 & -33\% & 0.429 & +210\% \\
& 192 & \textbf{0.141} & +9.6\% & 0.199 & +598\% & 0.177 & +19\% & 0.186 & +17\% & 0.451 & +9.0\% & 0.476 & +176\% \\
& 336 & \textbf{0.143} & +2.5\% & 0.195 & +613\% & 0.192 & +19\% & 0.190 & +11\% & 0.346 & +44\% & 0.377 & +260\% \\
& 720 & \textbf{0.215} & +30\% & 0.240 & +475\% & 0.234 & -1.7\% & 0.250 & +15\% & 0.348 &  +47\% & 0.773 & +171\%\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Weather$}} 
& 96 & 0.0073 & -38\% & 0.006  & -33\% & 0.006 & -23\% & 0.0070 & -17\% & \textbf{0.0022} & +167\% & 0.0065 &-11\%\\
& 192 & 0.0106 & -64\% & 0.007 & -14\% & 0.0074 & -11\% & \textbf{0.0063} & -19\% & 0.007 & -24\% & 0.0075 & -12\%\\
& 336 & 0.0079 & -37\% & 0.006 & +4.9\% & 0.0056 & +12\% & \textbf{0.0055} & +12\% & 0.0056 & +0.5\% & 0.222 & -69\% \\
& 720 &0.0063 & +0.4\% & 0.006 & +7.6\% & \textbf{0.0062} & +5.3\% & 0.103 & -36\% &0.006 & +4.2\% & 0.037 & -81\% \\
                        
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
& 24 & 1.393 &	+6.1\% & \textbf{1.220} & +36\% & 2.306 & +66\% & 4.189 & -9.2\% & 2.264 & -22\% & 2.249 & +217\% \\
& 36 & 1.242 & -22\% & \textbf{1.185} & +56\% & 2.950 & +44\% & 2.516 & +42\% & 1.841 & -3.0\% & 5.026 & +45\% \\
& 48 & 1.448 & -28\% & \textbf{1.079} & +79\% & 3.385 & +38\% & 3.501 & +16\% & 1.654 & +23\% & 2.838 & +115\% \\
& 60 & 2.089 & -18\% & \textbf{0.986} & +96\%  & 4.031 & +18\% & 4.258 & +10\% & 1.290 & +176\% & 4.978 & +250\% \\
\bottomrule
\end{tabular}
\label{tab:boosting}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%\end{wraptable}
%}


==> tables/tab_ablation_FEL.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[ht]
\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, and Transformer. S4 is also introduced as a variant. The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}&\multicolumn{2}{c}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.029} &\textbf{0.127}  &+0.0\%   & +0.0\%   & +12.1\% & +7.1\%    & +13.5\%   & +9.5\%   & +1.7\%  & +1.6\% &-- & -- \\
& 192  &\textbf{0.041} &\textbf{0.153}  &-1.5\% & -0.6\%  & +12.2\% & +8.5\%  & +10.8\%   & +7.8\%    & +2.0\%  & +3.3\% &-- & -- \\
& 336 & \textbf{0.053} & \textbf{0.175} &-1.7\% & -1.7\%  & +4.5\% & +4.0\%    & +10.8\%    & +6.3\%    & +4.5\% & +2.9\% &-- & --  \\
& 720 &\textbf{0.071}& \textbf{0.205}   &-0.9\%  & -1.0\%  & +5.5\% & +3.4\%  & +8.6\%    & +4.9\%    & +13.8\% & +7.8\% &-- & --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 

&96  &\textbf{0.154}  &\textbf{0.247}  &+155\%  & +81\%   & +160\% & +84\%    & +330\%  & +155\%  & +242\% & +119\% & 128\% & 83\% \\%&--& -- & \\
& 192 &\textbf{0.166} & \textbf{0.258} &+59\% & +39\%   & +121\%  & +67\%   & +224\%  & +117\%  & +264\% & +131\% & 124\% & 76\% \\%&--& --  \\
& 336 & \textbf{0.188}& \textbf{0.283} &+55\%  & +35\%   & +150\%  & +74\%   & +128\%  & +71\% & +183\% & +95\% & 117\% & 69\% \\%&--& -- \\
& 720 & \textbf{0.249}&\textbf{0.341}  &+33\%  & +25\%   & +154\%  & +73\%   & +192\%  & +95\%  & +312\% & +138\% & 89\% & 51\% \\ %&--& --  \\
                        
\bottomrule
\end{tabular}
\label{tab:ablation_FEL}
}
% \end{adjustwidth}
%\end{footnotesize}

\vskip -0.05in
\end{table*}
%}

==> tables/tab_ablation_FEL_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[!h]
\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{: (Full Benchmark)Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, and Transformer.The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}\vspace{-1mm}
\scalebox{0.8}{
\begin{tabular}{c|c|ccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& \\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.029} &\textbf{0.127}  &+0.0\%   & +0.0\%   & +12.1\% & +7.1\%    & +13.5\%   & +9.5\%   & +1.7\%  & +1.6\%  \\
& 192  &\textbf{0.041} &\textbf{0.153}  &-1.5\% & -0.6\%  & +12.2\% & +8.5\%  & +10.8\%   & +7.8\%    & +2.0\%  & +3.3\%  \\
& 336 & \textbf{0.053} & \textbf{0.175} &-1.7\% & -1.7\%  & +4.5\% & +4.0\%    & +10.8\%    & +6.3\%    & +4.5\% & +2.9\%   \\
& 720 &\textbf{0.071}& \textbf{0.205}   &-0.9\%  & -1.0\%  & +5.5\% & +3.4\%  & +8.6\%    & +4.9\%    & +13.8\% & +7.8\%   \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 

&96  &\textbf{0.154}  &\textbf{0.247}  &+155\%  & +81\%   & +160\% & +84\%    & +330\%  & +155\%  & +242\% & +119\%  \\%&--& -- & \\
& 192 &\textbf{0.166} & \textbf{0.258} &+59\% & +39\%   & +121\%  & +67\%   & +224\%  & +117\%  & +264\% & +131\%  \\%&--& --  \\
& 336 & \textbf{0.188}& \textbf{0.283} &+55\%  & +35\%   & +150\%  & +74\%   & +128\%  & +71\% & +183\% & +95\%  \\%&--& -- \\
& 720 & \textbf{0.249}&\textbf{0.341}  &+33\%  & +25\%   & +154\%  & +73\%   & +192\%  & +95\%  & +312\% & +138\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Exchange}} 

&96  &\textbf{0.110}  &\textbf{0.247}  &-13\%  & -12\%   & +51\% & +17\%    & +4.6\%  & -1.2\%  & -4.6\% & -5.8\%  \\%&--& -- & \\
& 192 &\textbf{0.207} & \textbf{0.352} &+7.2\% & +0.0\%   & +69\%  & +32\%   & +29\%  & +12\%  & +22\% & +11\%  \\%&--& --  \\
& 336 & \textbf{0.327}& \textbf{0.461} &+48\%  & +13\%   & +62\%  & +20\%   & +68\%  & +24\% & +72\% & +23\%  \\%&--& -- \\
& 720 & \textbf{0.811}&\textbf{0.708}  &+29\%  & +14\%   & +24\%  & +9.6\%   & +38\%  & +12\%  & +64\% & +27\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Traffic}} 

&96  &\textbf{0.144}  &\textbf{0.215}  &+69\%  & +47\%   & +13\% & +15\%    & +300\%  & +176\%  & +271\% & +161\%  \\%&--& -- & \\
& 192 &\textbf{0.120} & \textbf{0.199} &+17\% & +7.5\%   & +31\%  & +24\%   & +258\%  & +149\%  & +1572\% & +355\%  \\%&--& --  \\
& 336 & \textbf{0.128}& \textbf{0.212} &+6.2\%  & +7.6\%   & +16\%  & +15\%   & +151\%  & +102\% & +1514\% & +368\%  \\%&--& -- \\
& 720 & \textbf{0.153}&\textbf{0.252}  &+38\%  & +28\%   & +11\%  & +7.9\%   & +250\%  & +126\%  & +1048\% & +349\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 

&96  &\textbf{0.0012}  &\textbf{0.026}  &+17\%  & +6.2\%   & +16\% & +6.9\%    & +19\%  & +8.1\%  & +21\% & +8.9\%  \\%&--& -- & \\
& 192 &\textbf{0.0014} & \textbf{0.029} &-1.4\% & -2.4\%   & +5.0\%  & +1.7\%   & 0.7\%  & -0.7\%  & +4.3\% & +1.4\%  \\%&--& --  \\
& 336 & \textbf{0.0015}& \textbf{0.030} &+0.0\%  & -0.6\%   & +3.3\%  & +1.3\%   & +2.0\%  & +0.0\% & +3.3\% & +1.3\%  \\%&--& -- \\
& 720 & \textbf{0.0022}&\textbf{0.037}  &+4.6\%  & -0.3\%   & +4.1\%  & -1.6\%   & 3.6\%  & 0.0\%  & +0.0\% & -3.8\%  \\ %&--& --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{ILI}} 

&96  &\textbf{0.629}  &\textbf{0.538}  &+51\%  & +45\%   & -2.5\% & 9.5\%    & +20\%  & +29\%  & +112\% & +59\%  \\%&--& -- & \\
& 192 &\textbf{0.444} & \textbf{0.481} &+99\% & +58\%   & +25\%  & +24\%   & +84\%  & +56\%  & +360\% & +142\%  \\%&--& --  \\
& 336 & \textbf{0.557}& \textbf{0.584} &+33\%  & +31\%   & +21\%  & +16\%   & +58\%  & +30\% & +702\% & +94\%  \\%&--& -- \\
& 720 & \textbf{0.641}&\textbf{0.644}  &+8.4\%  & +5.4\%   & +23\%  & +18\%   & +42\%  & +22\%  & +74\% & +34\%  \\ %&--& --  \\
\bottomrule
\end{tabular}
\label{tab:ablation_FEL_full}
}
% \end{adjustwidth}
%\end{footnotesize}

\vskip -0.05in
\end{table*}
%}

==> tables/tab_ablation_FNO.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[ht]
\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, and Transformer. S4 is also introduced as a variant. The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}\vspace{-1mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}&\multicolumn{2}{c}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\midrule

\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030} &\textbf{0.128}  &+14\%   & +6.6\%   & +62\% & +31\%    & +286\%   & +118\%   & +709\%  & +166\% &-- & -- \\
& 192  &\textbf{0.047} &\textbf{0.160}  &+3.8\% & +2.2\%  & +271\% & +122\%  & +116\%   & +58\%    & +727\%  & +136\% &-- & -- \\
& 336 & \textbf{0.063} & \textbf{0.185} &-3.7\% & -2.1\%  & +90\% & +51\%    & +94\%    & +48\%    & +2524\% & +286\% &-- & --  \\
& 720 &\textbf{0.081}& \textbf{0.215}   &+0.9\%  & -0.6\%  & +127\% & +65\%  & +33\%    & +17\%    & +5783\% & +299\% &-- & --  \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
% &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

&96  &\textbf{0.213}  &\textbf{0.328}  &+103\%  & +40\%   & +37\% & +20\%    & +46\%  & +23\%  & +278\% & +105\% & 65\% & 38\% \\%&--& -- & \\
& 192 &\textbf{0.268} & \textbf{0.373} &+8.7\% & +0.01\%   & +32\%  & +14\%   & +42\%  & +21\%  & +249\% & +81\% & 39\% & 22\% \\%&--& --  \\
& 336 & \textbf{0.307}& \textbf{0.417} &-3.7\%  & -8.5\%   & +42\%  & +13\%   & +17\%  & +6.0\% & +564\% & +90\% & 33\% & 15\% \\%&--& -- \\
& 720 & \textbf{0.321}&\textbf{0.423}  &+5.7\%  & +1.4\%   & +98\%  & +36\%   & +32\%  & +18\%  & +2739\% & +117\% & 47\% & 22\% \\ %&--& --  \\
                        
                        
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} &96  & \textbf{0.079} & \textbf{0.204} &0.139 &0.276 &0.197  &0.323 &1.292 &0.849 &0.847  &0.752  &0.968  &0.812  &1.065  &0.829    \\
%                         & 192 & \textbf{0.159} & \textbf{0.292} &0.256 &0.369 &0.300  &0.369 &1.631 &0.968 &1.204   &0.895 &1.040  &0.851  &1.188  & 0.906   \\
%                         & 336 & \textbf{0.270} & \textbf{0.398} &0.426 &0.464 &0.509  &0.524 &2.225 &1.145 &1.672  &1.036  &1.659  &1.081  &1.357  &0.976     \\
%                         & 720 & \textbf{0.830} & \textbf{0.721} &1.090 &0.800 &1.447  &0.941 &2.521 &1.245 &2.478  &1.310  &1.941  &1.127  &1.510  &1.016     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Traffic$}} &96  &\textbf{0.453}& \textbf{0.305} &0.562 &0.349 &0.613  &0.388 &0.824 &0.514 &0.719  &0.391  &0.684  &0.384  &0.732  &0.423    \\
%                         & 192 & \textbf{0.463} & \textbf{0.308} &0.562 &0.346 &0.616&0.382 &1.106 &0.672 &0.696 &0.379  &0.685  &0.390  &0.733  &0.420    \\
%                         & 336 & \textbf{0.483} & \textbf{0.321} &0.570 &0.323 &0.622  &0.337 &1.084 &0.627 &0.777  &0.420  &0.733  &0.408  &0.742  &0.420     \\
%                         & 720 & \textbf{0.562} & 0.383 &0.596 &\textbf{0.368} &0.660  &0.408 &1.536 &0.845 &0.864  &0.472  &0.717  &0.396  &0.755  &0.423     \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Weather$}} & 96 & \textbf{0.199} & \textbf{0.262} &0.217  &0.296  &0.266  &0.336 &0.406 &0.444 &0.300  &0.384  &0.458  &0.490  &0.689  &0.596    \\
%                         & 192 & \textbf{0.228} & \textbf{0.288} &0.276  &0.336  &0.307  &0.367 &0.525 &0.527 &0.598  &0.544  &0.658  &0.589  &0.752  &0.638    \\
%                         & 336 &\textbf{0.267} &\textbf{0.323} & 0.339  &0.380  &0.359  &0.395 &0.531 &0.539 &0.578  &0.523  &0.797  &0.652  &0.639  &0.596    \\
%                         & 720 &\textbf{0.319} & \textbf{0.361} &0.403  &0.428 &0.578 &0.578 &0.419  &0.428  &1.059  &0.741  &0.869  &0.675  &1.130  &0.792    \\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ILI$}} & 24 & \textbf{1.970} & \textbf{0.875} &2.203  &0.963  &3.483 &1.287 &4.631 &1.484 &5.764  &1.677  &4.480  &1.444  &4.400 &1.382    \\
%                         & 36 & \textbf{1.982} & \textbf{0.859} &2.272  &0.976  &3.103  &1.148 &4.123 &1.348 &4.755  &1.467  &4.799  &1.467  &4.783  &1.448    \\
%                         & 48 & \textbf{1.868} & \textbf{0.896} &2.209  &0.981  &2.669  &1.085 &4.066 &1.36 &4.763  &1.469  &4.800  &1.468  &4.832  &1.465    \\
%                         & 60 & \textbf{2.057} & \textbf{0.929} &2.545  &1.061  &2.770  &1.125 &4.278 &1.41 &5.264  &1.564  &5.278  &1.560  &4.882  &1.483    \\
\bottomrule
\end{tabular}
\label{tab:ablation_FNO}
}
% \end{adjustwidth}
%\end{footnotesize}

\vskip -0.05in
\end{table*}
%}

==> tables/tab_ablation_HiPPO.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]

\vskip -0.05in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of LPU layer. The original LPU block (whose projection and reconstruction matrix are fixed) is replaced with 6 variants (\textbf{Fixed} means the matrix are not trainable. \textbf{Trainable} means the matrix is initialized with original parameters and trainable. \textbf{Random Init} means the matrix is initialized randomly and trainable). The experiments are performed on ETTm1 and Electricity with different input lengths. The metric of variants is presented in relative value (`+` indicates degraded performance, `-` indicates improved performance).}
\vspace{-1mm}
\resizebox{\columnwidth}{!}{
\scalebox{0.60}{

\begin{tabular}{c|c|cccccccccccccccccc}
\toprule

\multicolumn{2}{c|}{Index}&\multicolumn{2}{c|}{Original}&\multicolumn{2}{c|}{Variant 1}&\multicolumn{2}{c|}{Variant 2}&\multicolumn{2}{c|}{Variant 3}&\multicolumn{2}{c|}{Variant 4}&\multicolumn{1}{c|}{Variant 5}&\multicolumn{2}{c}{Variant 6}\\
\midrule

\multicolumn{2}{c|}{Projection}&\multicolumn{4}{c|}{Fixed}&\multicolumn{6}{c|}{Trainable}&\multicolumn{1}{c|}{Random Init}&\multicolumn{2}{c}{Linear}\\
\midrule
\multicolumn{2}{c|}{Reconstruction}&\multicolumn{2}{c|}{Fixed}&\multicolumn{2}{c|}{Trainable}&\multicolumn{2}{c|}{Fixed}&\multicolumn{2}{c|}{Trainable}&\multicolumn{2}{c|}{Random Init}&\multicolumn{1}{c|}{--}&\multicolumn{2}{c}{Linear}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& -- & MSE  & MAE \\
\midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
%                         & 192 & \textbf{0.240} & \textbf{0.313} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
%                         & 336 & \textbf{0.286} & \textbf{0.345} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
%                         & 720 & \textbf{0.393} & \textbf{0.410} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
% \midrule
\multirow{4}{*}{\rotatebox{90}{ETTm1}} 

&96  &\textbf{0.030} &\textbf{0.128}    &+6.0\%  & +3.1\% & +4.6\% & +3.1\%  & +4.7\%   & +2.7\%   & +0.7\% & +0.6\%  & NaN & +38\% & +22\%  \\
& 192  &\textbf{0.047} &\textbf{0.160}  &-2.6\%  & -1.3\%    & +2.5\% & +1.8\%  & -0.4\%   & +0.4\%   & -3.0\% & -1.0\%  & NaN  & +9.5\%  & +8.7\% \\
& 336 & \textbf{0.063} & \textbf{0.185} &+4.2\% & +1.8\%    & -2.4\% & -0.4\%  & -6.3\%   & -2.5\%    & +2.2\% & +1.4\%   & NaN & +5.8\% & +5.0\% \\
& 720 &\textbf{0.081}& \textbf{0.215}   &-0.4\%     & -0.6\%     &+24\%    & +12\%  & +11\%    & +5.9\%   & NaN & NaN       & NaN      & +1.4\%  & +2.2\% \\

\midrule

\multirow{4}{*}{\rotatebox{90}{Electricity}}
&96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% & +11\% & +4.8\%  &NaN & +136\% & +58\%  \\
& 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &NaN  & +32\%  & +16\% \\
& 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &NaN & +0.1\% & -5.0\% \\
& 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &NaN  & 37\%  & 22\% \\

\bottomrule
\end{tabular}
\label{tab:ablation_HiPPO}
}}
% \end{adjustwidth}
%\end{footnotesize}
\vskip -0.05in
\end{table*}

%}

==> tables/tab_ablation_normalize.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\vskip -0.15in
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of Normalization and Multiscale. Multiscale use 3 branches with: $T$, $2T$, and $4T$ as input sequence length. T is the predicted sequence length}\vspace{-1mm}
\scalebox{0.7}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Dataset}&\multicolumn{2}{c|}{ETTm2}&\multicolumn{2}{c|}{Electricity}&\multicolumn{2}{c|}{Exchange}&\multicolumn{2}{c|}{Traffic}&\multicolumn{2}{c|}{Weather}&\multicolumn{2}{c}{Illness}&\multicolumn{2}{c}{}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & Relative & MSE & Relative & MSE & Relative & MSE & Relative & MSE & Relative & MSE & Relative &\\
\midrule


\multirow{4}{*}{\rotatebox{90}{Methods}} 

&Original  &0.301 & +16\% & 0.195 & +4.8\% & 0.534 & + 60\% & 0.528 & +19\% & 0.264 & +4.9\% & 3.55 & + 80\% \\

& Normalization & 0.268 & +3.6\% & 0.199 & +6.4\% & 0.456 & +36\% & 0.656 & +48\% & 0.256 & +1.5\% & 3.36 & +70\% \\	
% &\textbf{0.047} &\textbf{0.160}  &-12\%  & -10\% & +2.5\% & +1.8\% & -0.4\%    & +0.4\%   & -\% & -\%  &--& --  \% \\
& Multiscale & 0.259 & + 0.19\% &	0.187 &   +0\%	& 0.335	 & 0\% & 0.541 & +22\% & 0.253 & +0.50\% &	2.41 & +22\% \\
& With both & 0.271	& +4.7\% &	0.189	& +1.5\% & 0.398 & +19\% & 0.442 & +0\% &  0.253 & +0.4\% & 1.97 & +0\% \\
% & 720 &\textbf{0.081}& \textbf{0.215}   &-0.\%     & -0.\%    & +\%    &  +\%   & +11\%    & +5.9\%   & -- & --       &--& - \\

% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
% % &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% % & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% % & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% % & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

% &96  &\textbf{0.213}  &\textbf{0.328}  &+100\%  & +100\%   & +37\% & +20\%    & +46\%  & +23\%  & +11\% & +4.8\%  \\%&--& -- & \\
% & 192 &\textbf{0.268} & \textbf{0.373} &+8.7\% & +0.01\%   & +32\%  & +14\%   & +42\%  & +21\%  & -5.3\% & -3.9\%  \\%&--& --  \\
% & 336 & \textbf{0.307}& \textbf{0.417} &-3.7\%  & -8.5\%   & +42\%  & +13\%   & +17\%  & +6.0\% & -8.5\% & -9.0\% \\%&--& -- \\
% & 720 & \textbf{0.321}&\textbf{0.423}  &+5.7\%  & +1.4\%   & +98\%  & +36\%   & +32\%  & +18\%  & +207\% & +85\% \\ %&--& --  \\
                        

\bottomrule
\end{tabular}
\label{tab:ablation_normalize}
}
\vskip -0.05in
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/tab_ett_m.tex <==

\begin{table*}[h]
\centering
% \begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Multivariate long-term forecasting results on ETT full benchmark. The best results are highlighted in bold. A lower MSE indicates better performance. All experiments are repeated 5 times.}
\vskip 0.05in
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
& 96 &\textbf{0.371} &\textbf{0.394} &0.376 &0.419  & 0.449& 0.459 &0.949 &0.777 & 0.865 & 0.713& 0.878& 0.740& 0.837& 0.728\\
& 192 &\textbf{0.414} &\textbf{0.423} &0.420 &0.448  & 0.500& 0.482 &0.882 &0.745 & 1.008 & 0.792& 1.037& 0.824& 0.923& 0.766\\
& 336 &\textbf{0.442} &\textbf{0.445} &0.459 &0.465  & 0.521& 0.496 &0.965 &0.75 & 1.107 & 0.809& 1.238& 0.932& 1.097& 0.835\\
& 720 &\textbf{0.465} &\textbf{0.472} &0.506 &0.507  & 0.514& 0.512 &1.074&0.814 & 1.181 &0.865&  1.135& 0.852& 1.257& 0.889\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
& 96  &\textbf{0.284} &\textbf{0.348} &0.346 &0.388 & 0.358& 0.397 &1.551&	0.968 & 3.755& 1.525& 2.116& 1.197 &2.626 &1.317\\
& 192 &\textbf{0.357} &\textbf{0.400} &0.429 &0.439 & 0.456& 0.452 &2.336	 &1.229 & 5.602& 1.931& 4.315& 1.635 &11.12 &2.979\\
& 336 &\textbf{0.377} &\textbf{0.417} &0.482 &0.480 & 0.482& 0.486 &2.801	 &1.259 & 4.721& 1.835& 1.124& 1.604 &9.323 &2.769\\
& 720 &\textbf{0.439} &\textbf{0.456} & 0.463 & 0.474 & 0.515& 0.511 &2.973	 &1.333 & 3.647& 1.625& 3.188& 1.540 &3.874 &1.697\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
& 96  &\textbf{0.302} &\textbf{0.345} &0.378 &0.418 & 0.505& 0.475 &0.640	 &0.584 & 0.672& 0.571& 0.600& 0.546 &0.538 &0.528\\
& 192 &\textbf{0.338} &\textbf{0.368} & 0.426 & 0.441 & 0.553& 0.496 &0.570	 &0.555 & 0.795& 0.669& 0.837& 0.700 &0.658 &0.592\\
& 336 &\textbf{0.373} &\textbf{0.388} & 0.445 & 0.459 & 0.621& 0.537 &0.795& 0.691& 1.212& 0.871& 1.124& 0.832 &0.898 &0.721\\
& 720 &\textbf{0.420} &\textbf{0.420} & 0.543 & 0.490 & 0.671& 0.561 &0.738 &0.655 & 1.166& 0.823& 1.153& 0.820 &1.102 &0.841\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 &\textbf{0.165} &\textbf{0.256} & 0.203 & 0.287 &0.255  &0.339  &0.705	 &0.690  &0.365  &0.453  &0.768  &0.642  &0.658  &0.619 \\
                        & 192 &\textbf{0.222} &\textbf{0.296} & 0.269 & 0.328 &0.281 &0.340  &0.924	 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827 \\
                        & 336 &\textbf{0.277} &\textbf{0.333} & 0.325 & 0.366  &0.339  &0.372  &1.364	 & 0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972 \\
                        & 720 &\textbf{0.371} &\textbf{0.389} & 0.421 & 0.415  &0.422  &0.419  &2.074 &1.074  &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242 \\
\bottomrule
\end{tabular}
}
\label{tab:multi-benchmarks-ett}
% \end{adjustwidth}
% \end{small}
% \vskip -0.1in
\end{table*}



==> tables/tab_ett_u.tex <==

\begin{table*}[h]
\centering
% \begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long-term forecasting results on ETT full benchmark. The best results are highlighted in bold. A lower MSE indicates better performance. All experiments are repeated 5 times.}
\vskip 0.05in
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{S4}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
&96 &\textbf{0.055}&\textbf{0.178}&0.079 &0.215 &0.071 &0.206 &0.316 &0.490 &	0.193&	0.377&	0.283&	0.468&	0.532&	0.569\\
&192 &\textbf{0.072}&\textbf{0.207}&0.104 &0.245 & 0.114&	0.262 & 0.345&0.516 &	0.217&	0.395&	0.234&	0.409&	0.568&	0.575\\
&336 &\textbf{0.083}&\textbf{0.229}&0.119 &0.270 &0.107&0.258 &0.825 &0.846 &	0.202&	0.381&	0.386&	0.546&	0.635&	0.589\\
&720 &\textbf{0.090}&\textbf{0.240}&0.127 &0.280 &0.126&0.283 &0.190 &0.355 &	0.183&	0.355&	0.475&	0.628&	0.762&	0.666\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
&96 &\textbf{0.127}&0.272&0.128 &\textbf{0.271} & 0.153&	0.306 & 0.381&0.501 &	0.213&	0.373&	0.217&	0.379&	1.411&	0.838\\
&192 &\textbf{0.182}&0.335&0.185 &\textbf{0.330} & 0.204&	0.351 & 0.332&0.458 &	0.227&	0.387&	0.281&	0.429&	5.658&	1.671\\
&336 &\textbf{0.204}&\textbf{0.367}&0.231 &0.378 & 0.246&	0.389 & 0.655&0.670 &	0.242&	0.401&	0.293&	0.437&	4.777&	1.582\\
&720 &\textbf{0.241}&\textbf{0.396}&0.278 &0.420 & 0.268&	0.409 & 0.630&0.662 &	0.291&	0.439&	0.218&	0.387&	2.042&	1.039\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
&96 &\textbf{0.029}&\textbf{0.127}&0.033 &0.140 & 0.056&	0.183 & 0.651&0.733 &	0.109&	0.277&	0.049&	0.171&	0.296&	0.355\\
&192 &\textbf{0.041}&\textbf{0.153}&0.058 &0.186 & 0.081&	0.216 & 0.190& 0.372&	0.151&	0.310&	0.157&	0.317&	0.429&	0.474\\
&336 &\textbf{0.053}&\textbf{0.175}&0.071 &0.209 & 0.076&	0.218 & 0.428&0.581 &	0.427&	0.591&	0.289&	0.459&	0.585&	0.583\\
&720 &\textbf{0.071}&\textbf{0.205}&0.102 &0.250 & 0.110&	0.267 & 0.254&0.433 &	0.438&	0.586&	0.430&	0.579&	0.782&	0.730\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 &0.065&\textbf{0.189}&\textbf{0.063} &0.189 & 0.065 & 0.189  & 0.153&0.318 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 &\textbf{0.094}&\textbf{0.233}& 0.102 & 0.245 & 0.118 & 0.256  &0.183 &0.350 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 &\textbf{0.124}&\textbf{0.274}& 0.130 & 0.279 & 0.154 & 0.305  &0.204 &0.367  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 &\textbf{0.173}&\textbf{0.323}& 0.178 & 0.325 & 0.182 &0.335  &0.482 &0.567  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-ett}
% \end{adjustwidth}
% \end{small}
\end{table*}

==> tables/tab_low_ran_approximation_full.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]

%\begin{wraptable}[9]{r}{0.6\textwidth}
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Low-rank Approximation (LRA) univariate forecasting study for frequency enhanced layer: Comp. K=0 means default version without LRA, 1 means the largest compression using K=1.}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Comp. K}&\multicolumn{2}{c|}{0}&\multicolumn{2}{c|}{16}&\multicolumn{2}{c|}{4}&\multicolumn{2}{c}{1}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.083  &0.209  &0.082  &0.208   &0.087    &0.217     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.166  &0.304  &0.166  &0.304   &0.172    &0.309      \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.340  &0.436  &0.300  &0.413   &0.349    &0.452      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &1.158  &0.806  &1.147  &0.801   &0.915   &0.719      \\
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 

&96&0.065&0.189&0.064&0.185&\textbf{0.064}&\textbf{0.185}&0.064&0.186 \\

&192&0.094&0.233&0.094&0.231&0.093&0.231&\textbf{0.093}&\textbf{0.231} \\

&336&0.124&0.274&0.124&0.270&\textbf{0.124}&\textbf{0.269}&0.124&0.271 \\

&720&0.173&0.323&0.173&0.322&\textbf{0.173}&\textbf{0.322}&0.177&0.328 \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 

&96&\textbf{0.154}&\textbf{0.247}&0.211&0.324&0.216&0.331&0.277&0.387 \\

&192&\textbf{0.166}&\textbf{0.258}&0.251&0.352&0.246&0.347&0.334&0.421 \\

&336&\textbf{0.188}&\textbf{0.283}&0.276&0.369&0.302&0.396&0.363&0.440 \\

&720&\textbf{0.249}&\textbf{0.341}&0.336&0.429&0.342&0.436&0.411&0.481 \\

\midrule

\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

&96&0.110&0.259&0.119&0.273&\textbf{0.104}&\textbf{0.247}&0.105&0.251 \\

&192&0.207&0.352&0.196&0.355&\textbf{0.195}&\textbf{0.349}&0.212&0.372 \\

&336&\textbf{0.327}&\textbf{0.461}&0.388&0.497&0.373&0.491&0.407&0.506 \\

&720&\textbf{0.811}&\textbf{0.708}&0.908&0.767&1.288&0.941&1.840&1.153 \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 

&96&\textbf{0.144}&\textbf{0.215}&0.146&0.223&0.154&0.237&0.267&0.373 \\

&192&\textbf{0.120}&\textbf{0.199}&0.121&0.201&0.138&0.231&0.218&0.333 \\

&336&0.128&0.212&\textbf{0.120}&\textbf{0.206}&0.132&0.227&0.216&0.335 \\

&720&\textbf{0.153}&\textbf{0.252}&0.155&0.257&0.154&0.257&0.246&0.366 \\

\midrule

\multirow{4}{*}{\rotatebox{90}{$Weather$}} 

&96&0.0012&0.026&0.0011&0.025&\textbf{0.001}&\textbf{0.025}&0.001&0.025 \\

&192&0.0014&0.029&0.0014&0.028&\textbf{0.001}&\textbf{0.028}&0.001&0.028 \\

&336&0.0015&0.03&0.0015&0.030&\textbf{0.001}&\textbf{0.029}&0.002&0.030 \\

&720&0.0022&0.037&0.0022&0.037&\textbf{0.002}&\textbf{0.037}&0.002&0.037 \\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ILI$}} 

&96&0.629&0.538&\textbf{0.599}&\textbf{0.556}&0.628&0.558&0.630&0.579 \\

&192&\textbf{0.444}&\textbf{0.481}&0.487&0.533&0.508&0.561&0.570&0.612 \\

&336&0.557&0.584&\textbf{0.553}&\textbf{0.565}&0.703&0.696&0.722&0.706 \\

&720&\textbf{0.641}&\textbf{0.644}&0.648&0.641&0.900&0.780&1.493&1.032 \\

\midrule
\multicolumn{2}{c|}{Parameter size}&\multicolumn{2}{c|}{100\%}&\multicolumn{2}{c|}{6.4\%}&\multicolumn{2}{c|}{1.6\%}&\multicolumn{2}{c}{0.4\%}\\
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:FEL_LRA_FULL}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%\end{wraptable}
%}

==> tables/tab_low_rank_approximation.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]

%\begin{wraptable}[9]{r}{0.6\textwidth}
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Low-rank Approximation (LRA) study for frequency enhanced layer: Comp. K=0 means default version without LRA, 1 means the largest compression using K=1.}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Comp. K}&\multicolumn{2}{c|}{0}&\multicolumn{2}{c|}{16}&\multicolumn{2}{c|}{4}&\multicolumn{2}{c}{1}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.083  &0.209  &0.082  &0.208   &0.087    &0.217     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.166  &0.304  &0.166  &0.304   &0.172    &0.309      \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.340  &0.436  &0.300  &0.413   &0.349    &0.452      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &1.158  &0.806  &1.147  &0.801   &0.915   &0.719      \\
\multirow{4}{*}{\rotatebox{90}{$ETTh1$}} 

&96  &\textbf{0.371} &\textbf{0.394}    &0.371  &0.397  &0.373  &0.399   & 0.391   & 0.418    \\
& 192  &0.414 &\textbf{0.423}  &0.414  &0.425  &\textbf{0.413}  &0.426   &  0.437  &  0.445    \\
& 336 & \textbf{0.442} & 0.445 &0.452  &0.451  &0.445  &\textbf{0.444}   &0.460    &0.458       \\
& 720 &\textbf{0.454}& \textbf{0.451}   &0.460  &0.472  &0.461  &0.471   &0.464    &0.476      \\

\midrule

\multirow{4}{*}{\rotatebox{90}{$Weather$}} 

&96  &\textbf{0.199} &\textbf{0.262}    &0.200  &0.266  &0.199  &0.263   &0.198    &0.261      \\
& 192  &0.228 &0.288  &0.232  &0.298  &0.227  &0.287   &\textbf{0.226}    &\textbf{0.285}       \\
& 336 & 0.267 & 0.323 &0.266  &0.320  &\textbf{0.253}  &\textbf{0.314}   &0.264    &0.316       \\
& 720 &0.319& 0.361   &\textbf{0.314}  &\textbf{0.352}  &0.319  &0.361   &0.314    &0.354      \\

\midrule
\multicolumn{2}{c|}{Parameter size}&\multicolumn{2}{c|}{100\%}&\multicolumn{2}{c|}{6.4\%}&\multicolumn{2}{c|}{1.6\%}&\multicolumn{2}{c}{0.4\%}\\
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:FEL_LRA}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%\end{wraptable}
%}

==> tables/tab_lra_3d.tex <==
%\resizebox{!}{\.5\paperheight}{

% \begin{wraptable}[11]{r}{0.6\textwidth}
\vskip -0.15in
% \begin{wraptable}{r}{0.6\textwidth}
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Low-rank Approximation (LRA) study for Frequency Enhanced Layer (FEL): Comp. K=0 means default version without LRA, 1 means the largest compression using K=1.}\vspace{-1.5mm}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccc}
\toprule

\multicolumn{2}{c|}{Comp. K}&\multicolumn{2}{c|}{0}&\multicolumn{2}{c|}{16}&\multicolumn{2}{c|}{4}&\multicolumn{2}{c}{1}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.083  &0.209  &0.082  &0.208   &0.087    &0.217     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.166  &0.304  &0.166  &0.304   &0.172    &0.309      \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.340  &0.436  &0.300  &0.413   &0.349    &0.452      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &1.158  &0.806  &1.147  &0.801   &0.915   &0.719      \\
\multirow{4}{*}{\rotatebox{90}{ETTh1}} 

&96  &\textbf{0.371} &\textbf{0.394}    &0.371  &0.396  &0.371  &0.398   & 0.400   & 0.421    \\
& 192  &0.414 &\textbf{0.423}  &0.411  &0.423  &0.414  &0.426   & 0.435   & 0.444    \\
& 336 & \textbf{0.442} & 0.445 &0.443  &0.446  &0.443  & 0.444  & 0.492   &  0.478     \\
& 720 &\textbf{0.454}& \textbf{0.451}   &0.464  &0.474  &0.468  &0.478   & 0.501   & 0.499      \\

\midrule

\multirow{4}{*}{\rotatebox{90}{Weather}} 
&96  &\textbf{0.199} &\textbf{0.262}   &0.199  &0.263  &0.197  &0.262   &0.198    & 0.263     \\
& 192  &0.228 &0.288  &0.225  &0.285  &0.226  &0.285   &0.225    & 0.286      \\
& 336 & 0.267 & 0.323 &0.266  &0.321  &0.263  &0.314   & 0.264   &  0.316      \\
& 720 &0.319& 0.361  &0.314 &0.355  &0.315  & 0.354   &0.318    & 0.357   \\
\midrule
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 

% &96  &\textbf{0.079} &\textbf{0.204}    &0.079  &0.202  &0.081  &0.206   &0.084    &0.211     \\
% & 192  &\textbf{0.159} &\textbf{0.292}  &0.152  &0.287  &0.163  &0.299   &0.176    &0.313     \\
% & 336 & \textbf{0.270} & \textbf{0.398} &0.301  &0.411  &0.340  &0.439   &0.368    &0.459      \\
% & 720 &\textbf{0.788}& \textbf{0.680}   &0.952  &0.726  &1.229  &0.833   &1.705    &1.021     \\
% \midrule

\multicolumn{2}{c|}{Parameter size}&\multicolumn{2}{c|}{100\%}&\multicolumn{2}{c|}{1.95\%}&\multicolumn{2}{c|}{0.41\%}&\multicolumn{2}{c}{0.10\%}\\
% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:FEL_LRA}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
% \end{wraptable}
%}

==> tables/tab_mean_std.tex <==
\vspace{-.2cm}
\begin{table}[ht]
%\setlength{\uppercaptionskip}{0.pt}
%\setlength{\belowcaptionskip}{-0.pt}
% \label{sample-table-kstest}
%\vskip 0.15in
\centering
% \setlength{\belowcaptionskip}{2pt} 
\caption{MSE with error bars (Mean and STD) for FiLM and FEDformer baseline for multivariate long-term forecasting. All experiments are repeated 5 times.}
\begin{small}
% \begin{sc}
\scalebox{0.75}{
\begin{tabular}{c|c|ccccc}
\toprule
\multicolumn{2}{c|}{MSE}& ETTm2 & Electricity & Exchange & Traffic\\ %&\multicolumn{2}{c|}{Fedformer-f }\\%&\multicolumn{2}{c|}{}&\\
\midrule
\multirow{4}{*}{\rotatebox{90}{FiLM}} 
& 96 & 0.165 $\pm$ 0.0051 & 0.153$\pm$ 0.0014 & 0.079$\pm$ 0.002 & 0.416$\pm$ 0.010 \\
& 192 & 0.222 $\pm$ 0.0038 & 0.165$\pm$ 0.0023 & 0.159$\pm$ 0.011 & 0.408$\pm$ 0.007 \\
& 336 & 0.277 $\pm$ 0.0021 & 0.186$\pm$ 0.0018 & 0.270$\pm$ 0.018 & 0.425$\pm$ 0.007 \\
& 720 & 0.371 $\pm$ 0.0066 & 0.236$\pm$ 0.0022 & 0.536$\pm$ 0.026 & 0.520$\pm$ 0.003 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{FED-f}} 
& 96 & 0.203 $\pm$ 0.0042 & 0.194 $\pm$ 0.0008 & 0.148 $\pm$ 0.002 & 0.217 $\pm$ 0.008 \\
& 192 & 0.269 $\pm$ 0.0023 & 0.201$\pm$ 0.0015 & 0.270$\pm$ 0.008 & 0.604 $\pm$ 0.004 \\
& 336 & 0.325 $\pm$ 0.0015 & 0.215$\pm$ 0.0018 & 0.460$\pm$ 0.016 & 0.621 $\pm$ 0.006 \\
& 720 & 0.421 $\pm$ 0.0038 & 0.246$\pm$ 0.0020 & 1.195$\pm$ 0.026 & 0.626 $\pm$ 0.003 \\
\bottomrule
\end{tabular}
}
\label{tab:std}
% \end{sc}
\end{small}
%\end{center}
\vskip -0.1in
\end{table}




==> tables/tab_mode_selection_policy.tex <==
% \begin{wraptable}[16]{r}{0.6\textwidth}
\begin{table*}[h]

% \begin{wraptable}[11]{r}{0.5\textwidth}
\vskip -0.1in

\centering
\caption{Mode selection policy study for frequency enhanced layer. Lowest: select the lowest $m$ frequency mode; Random: select $m$ random frequency mode; Low random: select the $0.8*m$ lowest frequency mode and $0.2*m$ random high frequency mode.}\vspace{-1.5mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccc}
\toprule
\multicolumn{2}{c|}{Policy}&\multicolumn{2}{c|}{Lowest}&\multicolumn{2}{c|}{Random}&\multicolumn{2}{c}{Low random}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE \\
\midrule

\multirow{4}{*}{\rotatebox{90}{Exchange}} 

&96  &\textbf{0.086} &\textbf{0.204}    &0.086  &0.208  &0.087  &0.210        \\
& 192  &0.188 &\textbf{0.292}  &\textbf{0.187}  &0.318  &0.207  &0.340      \\
& 336 & 0.356 & \textbf{0.433} &0.358  &0.437  &\textbf{0.353}  &0.461   \\
& 720 &\textbf{0.727}& \textbf{0.669}   &0.788  &0.680  &0.748  &0.674   \\

\midrule

\multirow{4}{*}{\rotatebox{90}{Weather}} 

&96  &0.199 &0.262 &0.197  &0.256  &\textbf{0.196}  &\textbf{0.254}   \\
& 192  &\textbf{0.228} &\textbf{0.288}  &0.234  &0.300  &0.234  &0.301   \\
& 336 & 0.267 & 0.323 &0.266  &0.319  &\textbf{0.263}  &\textbf{0.316}   \\
& 720 &0.319& 0.361 &0.317  &0.356  &\textbf{0.316}  &\textbf{0.354}  \\

\bottomrule

\end{tabular}
\label{tab:mode}
}
\end{table*}
% \end{wraptable}


==> tables/tab_mode_selection_policy_full.tex <==
% \begin{wraptable}[16]{r}{0.6\textwidth}
\begin{table*}[h]

% \begin{wraptable}[11]{r}{0.5\textwidth}
\vskip -0.1in

\centering
\caption{Mode selection policy study for frequency enhanced layer. Lowest: select the lowest $m$ frequency mode; Random: select $m$ random frequency mode; Low random: select the $0.8*m$ lowest frequency mode and $0.2*m$ random high frequency mode.}\vspace{-1.5mm}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccc}
\toprule
\multicolumn{2}{c|}{Policy}&\multicolumn{2}{c|}{Lowest}&\multicolumn{2}{c|}{Random}&\multicolumn{2}{c}{Low random}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE \\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} 
&96&\textbf{0.065}&\textbf{0.189}&0.066&0.189&0.066&0.190 \\

&192&\textbf{0.094}&\textbf{0.233}&0.096&0.235&0.096&0.235 \\

&336&\textbf{0.124}&0.274&0.125&\textbf{0.270}&0.128&0.275 \\

&720&0.173&0.323&\textbf{0.173}&\textbf{0.322}&0.173&0.323 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} 
&96&\textbf{0.154}&\textbf{0.247}&0.175&0.0.260&0.176&0.262 \\

&192&\textbf{0.166}&\textbf{0.258}&0.177&0.266&0.168&0.273 \\

&336&\textbf{0.188}&\textbf{0.283}&0.199&0.289&0.192&0.299 \\

&720&\textbf{0.249}&\textbf{0.341}&0.269&0.364&0.270&0.362 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Exchange}} 
&96&0.11&0.259&0.110&0.256&\textbf{0.106}&\textbf{0.249} \\

&192&0.207&0.352&\textbf{0.196}&\textbf{0.351}&0.207&0.357 \\

&336&\textbf{0.327}&\textbf{0.461}&0.451&0.522&0.373&0.484 \\

&720&0.811&0.708&0.835&0.714&\textbf{0.604}&\textbf{0.628} \\


\midrule
\multirow{4}{*}{\rotatebox{90}{Traffic}} 
&96&\textbf{0.144}&\textbf{0.215}&0.145&0.216&0.145&0.217 \\

&192&0.12&0.199&0.119&0.198&\textbf{0.118}&\textbf{0.197} \\

&336&0.128&0.212&\textbf{0.122}&\textbf{0.207}&0.122&0.209 \\

&720&0.153&0.252&\textbf{0.142}&\textbf{0.238}&0.155&0.259 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{Weather}} 
&96&\textbf{0.0012}&\textbf{0.026}&0.0012&0.027&0.0012&0.026 \\

&192&\textbf{0.0014}&\textbf{0.029}&0.0014&0.029&0.0014&0.029 \\

&336&\textbf{0.0015}&\textbf{0.03}&0.0015&0.030&0.0015&0.030 \\

&720&\textbf{0.0022}&\textbf{0.037}&0.0023&0.037&0.0023&0.037 \\

\midrule
\multirow{4}{*}{\rotatebox{90}{ILI}} 
&96&0.629&0.538&0.639&0.542&\textbf{0.626}&\textbf{0.537} \\

&192&\textbf{0.444}&\textbf{0.481}&0.448&0.490&0.447&0.494 \\

&336&\textbf{0.557}&\textbf{0.584}&0.560&0.590&0.557&0.587 \\

&720&\textbf{0.641}&\textbf{0.644}&0.641&0.647&0.643&0.650 \\



\bottomrule

\end{tabular}
\label{tab:mode_full}
}
\end{table*}
% \end{wraptable}


==> tables/tab_noise_injection.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Noise injection studies. A 0.3*$\mathcal{N}\left(0,1\right)$ Gaussian noise is introduced into our training/testing. We conduct 4 sets of experiments with/without noise in training and test phases. The experiments are performed on ETTm1 and Electricity with different output lengths. The metric of variants is presented in relative value ('+' indicates degraded performance, and '-' indicates improved performance).}
%\resizebox{\columnwidth}{!}{
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccc}
\toprule

\multicolumn{2}{c|}{Training}&\multicolumn{4}{c|}{noise}&\multicolumn{4}{c}{with noise}\\
\midrule
\multicolumn{2}{c|}{Testing}&\multicolumn{2}{c|}{without noise}&\multicolumn{2}{c|}{with noise}&\multicolumn{2}{c|}{without noise}&\multicolumn{2}{c}{with noise}\\

\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE \\
\midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
%                         & 192 & \textbf{0.240} & \textbf{0.313} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
%                         & 336 & \textbf{0.286} & \textbf{0.345} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
%                         & 720 & \textbf{0.393} & \textbf{0.410} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
% \midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh1$}} 

&96  &\textbf{0.371} &\textbf{0.394}    &-1.6\%  & -2.0\% & -0.0\% & -0.0\%  & -1.6\%   & -2.0\%     \\
& 192  &\textbf{0.414} &\textbf{0.423}  &-0.5\%  & -1.4\%    & +0.5\% & -0.0\%  & -0.5\%   & -1.4\%    \\
& 336 & \textbf{0.442} & \textbf{0.445} &-1.8\% & -0.9\%    & -0.9\% & +1.3\%  & -3.2\%   & -1.6\%     \\
& 720 &\textbf{0.465}& \textbf{0.472}   &+0.2\%     & -0.2\%     &+0.9\%    & +0.9\%  & -0.6\%    & -0.4\%    \\

% \midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}}
% &96  &\textbf{0.079}  &\textbf{0.204}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.1\% \\
% & 192 &\textbf{0.159} & \textbf{0.292} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\%  \\
% & 336 & \textbf{0.270}& \textbf{0.398}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\% \\
% & 720 & \textbf{0.830}&\textbf{0.721} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\% \\
\bottomrule
\end{tabular}
\label{tab:ablation_noise}
}
%}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/tab_parameter_size.tex <==
\begin{table}[h]
\centering
% \setlength{\belowcaptionskip}{2pt} 
\caption{Parameter size of baseline models and FiLM with different low-rank approximations: the models are trained and tested on ETT dataset; the subscript number denotes $k$ in low-rank approximation.}
\begin{small}
% \begin{sc}
\vskip 0.05in
\begin{tabular}{c|ccccccc}
\toprule
Methods&Transformer&Autoformer&FEDformer&FiLM&$\mathrm{FiLM}_{16}$ & $\mathrm{FiLM}_4$ & $\mathrm{FiLM}_1$\\
\midrule
Parameter(M) & 0.0069 & 0.0069& 0.0098& 1.50 & 0.0293 &0.0062& 0.00149 \\
%&\multicolumn{2}{c|}{Fedformer-f }\\%&\multicolumn{2}{c|}{}&\\
\bottomrule
\end{tabular}
\label{tab:size}
% \end{sc}
\end{small}
%\end{center}
\vskip -0.1in
\end{table}


==> tables/tab_rebuttal_nhits.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h!]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{multivariate long-term series forecasting results on six datasets with various input length and prediction length $O \in \{96,192,336,720\}$ (For ILI dataset, we set prediction length $O \in \{24,36,48,60\}$). Supplementary results of non-Transformer baselines (N-Hits and a seasonal-naive model).}
% \vspace{-1mm}
\scalebox{0.8}{
\begin{tabular}{c|c|cccccccccccccccc|}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{N-Hits}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Seasonal-naive}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
                        &96 & \textbf{0.165} & 0.256 & 0.176 & \textbf{0.255} &0.203 &0.287 &0.255  &0.339  &0.262 &0.300 \\
                        & 192 & \textbf{0.222} & \textbf{0.296} & 0.245 & 0.305 & 0.269  &0.328  &0.281 &0.340  &0.319 &0.337\\
                        & 336 & \textbf{0.277} & \textbf{0.333} & 0.295 & 0.346 & 0.325 &0.366 &0.339  &0.372  &0.375 &0.371\\
                        & 720 & \textbf{0.371} & \textbf{0.389} & 0.401 & 0.426 & 0.421 &0.415 &0.422  &0.419 &0.469 &0.422\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
                        &96  &0.154  &0.267 & \textbf{0.147} & \textbf{0.249}  &0.183 &0.297 &0.201  &0.317 &0.211 &0.278\\
                        & 192 &\textbf{0.164} & \textbf{0.258} & 0.167 & 0.269 & 0.195 &0.308 &0.222  &0.334 &0.214 &0.282\\
                        & 336 & 0.188 & \textbf{0.283} & \textbf{0.186} & 0.290 & 0.212 &0.313 &0.231 &0.338 &0.226 &0.294\\
                        & 720 & 0.236 & \textbf{0.332} & 0.243 & 0.340 &\textbf{0.231} &0.343 &0.254  &0.361 &0.265 & 0.324\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
                        &96  & \textbf{0.086} & \textbf{0.204} &0.092 & 0.211 & 0.139 & 0.276 & 0.197 &0.323 &0.086 &0.204 \\
                        & 192 & \textbf{0.189} & \textbf{0.292} & 0.208 & 0.322 &0.256 &0.369 & 0.300 & 0.369 &0.172 &0.295\\
                        & 336 & \textbf{0.356} & \textbf{0.433} & 0.371 & 0.443 & 0.426 &0.464 & 0.509 & 0.524 &0.311 &0.401\\
                        & 720 & \textbf{0.727} & \textbf{0.669} & 0.888 & 0.723 &  1.090 &0.800 & 1.447 & 0.941 &0.832 &0.686\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
                        &96  & 0.416& 0.294 & \textbf{0.402} & \textbf{0.282} & 0.562 &0.349 &0.613  &0.388 &1.219 &0.497\\
                        & 192 & \textbf{0.408} & \textbf{0.288} &0.420 & 0.297 & 0.562 &0.346 &0.616&0.382 &1.089 &0.456\\
                        & 336 & \textbf{0.425} & \textbf{0.298} &0.448 & 0.313 & 0.570 &0.323 &0.622  &0.337 &1.147 &0.473\\
                        & 720 & \textbf{0.520} &\textbf{0.353} &0.539 & 0.353 & 0.596 &0.368 &0.660  &0.408 &1.181 &0.486\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$Weather$}} 
                        & 96 & 0.199 & 0.262 & \textbf{0.158} & \textbf{0.195} & 0.217  &0.296  &0.266  &0.336 &0.315 &0.288\\
                        & 192 & 0.228 & 0.288 & \textbf{0.211} & \textbf{0.247} & 0.276  &0.336  &0.307  &0.367 &0.341 &0.305\\
                        & 336 &\textbf{0.267} & 0.323 & 0.274 & \textbf{0.300} & 0.339  &0.380  &0.359  &0.395 &0.381 &0.331\\
                        & 720 &\textbf{0.319} & 0.361 &0.351 & \textbf{0.353} & 0.403  &0.428 &0.578 &0.578 &0.440 &0.370 \\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ILI$}} 
                        & 24 & 1.970 & 0.875 & \textbf{1.862} & \textbf{0.869} & 2.203  &0.963  &3.483 &1.287 &6.581 &1.699 \\
                        & 36 & \textbf{1.982} & \textbf{0.859} &2.071 & 0.969 & 2.272  &0.976  &3.103  &1.148 &7.121 &1.882 \\
                        & 48 & \textbf{1.868} & \textbf{0.896} &2.346 & 1.042 & 2.209  &0.981  &2.669  &1.085 &6.567 &1.797 \\
                        & 60 & \textbf{2.057} & \textbf{0.929} &2.560 & 1.073 & 2.545  &1.061  &2.770  &1.125 &5.885 &1.675 \\
\bottomrule
\end{tabular}
\label{tab:multi-benchmarks}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}


% %\resizebox{!}{\.5\paperheight}{
% % \vskip -0.2in
% \begin{table*}[h]
% \centering
% %\begin{footnotesize}
% % \begin{adjustwidth}{-1.5in}{-1in}
% \caption{Univariate Benchmark}
% % \vspace{-1mm}
% \scalebox{0.8}{
% \begin{tabular}{c|c|cccccccccccccc|}
% \toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM}&\multicolumn{2}{c|}{N-Hits}&\multicolumn{2}{c|}{N-BEATS}&\multicolumn{2}{c|}{FEDformer}&\multicolumn{2}{c|}{Autoformer}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE & MSE  & MAE\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
% & 96 & 0.065 & 0.189  & 0.066 & \textbf{0.185} & 0.082 & 0.219 &\textbf{0.063} &0.189 & 0.065 & 0.189 \\
% & 192& 0.094 & 0.233 & \textbf{0.087} & \textbf{0.223} & 0.120 & 0.268 &0.102 &0.245 & 0.118 & 0.256 \\
% & 336 & 0.124 & \textbf{0.274} & \textbf{0.106} &0.251&0.226 & 0.370& 0.130 &0.279 & 0.154 & 0.305  \\
% & 720 & \textbf{0.173} & 0.323 &0.178 &\textbf{0.312} &0.188 & 0.338 & 0.312&0.325 & 0.182 &0.335 \\
% \midrule

% \multirow{4}{*}{\rotatebox{90}{$Exchange$}} 
% &96  & 0.110 & 0.259 & \textbf{0.093} & \textbf{0.223} & 0.156 & 0.299 & 0.131 &0.284 & 0.241 & 0.387\\
% & 192 & \textbf{0.207} & 0.352& 0.230 & \textbf{0.313} &0.669  &0.665& 0.277 &0.420  &0.300  &0.369 \\
% & 336 & \textbf{0.327} & \textbf{0.461} &0.370 &0.486 &0.611 &0.605 &0.486&0.511 &0.509  &0.524 \\
% & 720 & 0.811 & 0.708 &\textbf{0.728} & \textbf{0.569}& 1.111 &0.860& 1.162 &0.832 &1.260  &0.867 \\
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$Traffic$}} 
% %                         &96  & 0.416& 0.294 & \textbf{0.402} & \textbf{0.282} & 0.562 &0.349 &0.613  &0.388 \\
% %                         & 192 & \textbf{0.408} & \textbf{0.288} &0.420 & 0.297 & 0.562 &0.346 &0.616&0.382\\
% %                         & 336 & \textbf{0.425} & \textbf{0.298} &0.448 & 0.313 & 0.570 &0.323 &0.622  &0.337\\
% %                         & 720 & \textbf{0.520} &\textbf{0.353} &0.539 & 0.353 & 0.596 &0.368 &0.660  &0.408 \\
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$Weather$}} 
% %                         & 96 & 0.199 & 0.262 & \textbf{0.158} & \textbf{0.195} & 0.217  &0.296  &0.266  &0.336\\
% %                         & 192 & 0.228 & 0.288 & \textbf{0.211} & \textbf{0.247} & 0.276  &0.336  &0.307  &0.367\\
% %                         & 336 &\textbf{0.267} & 0.323 & 0.274 & \textbf{0.300} & 0.339  &0.380  &0.359  &0.395 \\
% %                         & 720 &\textbf{0.319} & 0.361 &0.351 & \textbf{0.353} & 0.403  &0.428 &0.578 &0.578 \\
% % \midrule
% % \multirow{4}{*}{\rotatebox{90}{$ILI$}} 
% %                         & 24 & 1.970 & 0.875 & \textbf{1.862} & \textbf{0.869} & 2.203  &0.963  &3.483 &1.287 \\
% %                         & 36 & \textbf{1.982} & \textbf{0.859} &2.071 & 0.969 & 2.272  &0.976  &3.103  &1.148 \\
% %                         & 48 & \textbf{1.868} & \textbf{0.896} &2.346 & 1.042 & 2.209  &0.981  &2.669  &1.085 \\
% %                         & 60 & \textbf{2.057} & \textbf{0.929} &2.560 & 1.073 & 2.545  &1.061  &2.770  &1.125 \\
% \bottomrule
% \end{tabular}
% \label{tab:multi-benchmarks}
% }
% % \end{adjustwidth}
% %\end{footnotesize}
% \end{table*}
%}

==> tables/tab_signal_recovery.tex <==
%\resizebox{!}{\.5\paperheight}{
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Ablation studies of FEL layer. The FEL layer is replaced with 4 different variants: MLP, LSTM, CNN, Transformer. S4 is also introduced as a variant. The experiments are performed on ETTm1 and Electricity. The metric of variants is presented in relative value (’+’ indicates degraded performance, ’-’ indicates improved performance).}
\scalebox{0.75}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FilM}&\multicolumn{2}{c|}{LPU+MLP}&\multicolumn{2}{c|}{LPU+LSTM}&\multicolumn{2}{c|}{LPU+CNN}&\multicolumn{2}{c|}{LPU+attention}&\multicolumn{2}{c}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE&\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ETTm1$}} 

&96  &\textbf{0.030} &\textbf{0.128}  &+14\%   & +6.6\%   & +62\% & +31\%    & +286\%   & +118\%   & +709\%  & +166\% &-- & -- \\
% & 192  &\textbf{0.047} &\textbf{0.160}  &+3.8\% & +2.2\%  & +271\% & +122\%  & +116\%   & +58\%    & +727\%  & +136\% &-- & -- \\
% & 336 & \textbf{0.063} & \textbf{0.185} &-3.7\% & -2.1\%  & +90\% & +51\%    & +94\%    & +48\%    & +2524\% & +286\% &-- & --  \\
% & 720 &\textbf{0.081}& \textbf{0.215}   &+0.9\%  & -0.6\%  & +127\% & +65\%  & +33\%    & +17\%    & +5783\% & +299\% &-- & --  \\

% \midrule
% \multirow{4}{*}{\rotatebox{90}{$Electricity$}} 
% % &96  &\textbf{0.213}  &\textbf{0.328}  &+15\%  & +6.8\% & +11\% & +5.2\%  & +11\%    & +5.2\% & +11\% & +4.8\%  &--& -- & +136\% & +58\%  \\
% % & 192 &\textbf{0.268} & \textbf{0.373} &-4.6\% & -3.8\% & +7.8\%  & +3.9\%   & +6.8\%    & +3.5\% & -5.3\% & -3.9\%  &--& --  & +32\%  & +16\% \\
% % & 336 & \textbf{0.307}& \textbf{0.417}&-4.2\%  & -5.0\% & -3.9\%  & -6.0\%   & -7.2\%    & -8.0\%   & -8.5\% & -9.0\%   &--& -- & +0.1\% & -5.0\% \\
% % & 720 & \textbf{0.321}&\textbf{0.423} &+2.9\%  & +2.8\% & +10\%  &  +6.8\%  & +3.0\%   & +1.7\%  & +207\% & +85\%      &--& --  & 37\%  & 22\% \\

% &96  &\textbf{0.213}  &\textbf{0.328}  &+103\%  & +40\%   & +37\% & +20\%    & +46\%  & +23\%  & +278\% & +105\% & 65\% & 38\% \\%&--& -- & \\
% & 192 &\textbf{0.268} & \textbf{0.373} &+8.7\% & +0.01\%   & +32\%  & +14\%   & +42\%  & +21\%  & +249\% & +81\% & 39\% & 22\% \\%&--& --  \\
% & 336 & \textbf{0.307}& \textbf{0.417} &-3.7\%  & -8.5\%   & +42\%  & +13\%   & +17\%  & +6.0\% & +564\% & +90\% & 33\% & 15\% \\%&--& -- \\
% & 720 & \textbf{0.321}&\textbf{0.423}  &+5.7\%  & +1.4\%   & +98\%  & +36\%   & +32\%  & +18\%  & +2739\% & +117\% & 47\% & 22\% \\ %&--& --  \\
                        
                        
\bottomrule
\end{tabular}
\label{tab:ablation_FNO}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}

==> tables/useless_tabs/tab_hyperparam.tex <==

\begin{table*}[h]
\centering
% \begin{small}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Univariate long sequence time-series forecasting results on ETTm1, parameter sensitivity}
\vskip 0.05in
\scalebox{0.85}{
\begin{tabular}{c|c|cccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer-f}&\multicolumn{2}{c|}{FEDformer-w}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule

\multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
&96 &0.079 &0.215 &0.080 &0.214 &\textbf{0.071} &\textbf{0.206}&	0.193&	0.377&	0.283&	0.468&	0.532&	0.569\\
&192 &\textbf{0.104} &\textbf{0.245} &0.105 &0.256 & 0.114&	0.262&	0.217&	0.395&	0.234&	0.409&	0.568&	0.575\\
&336 &0.119 &0.270 &0.120 &0.269 &\textbf{0.107}&\textbf{0.258}&	0.202&	0.381&	0.386&	0.546&	0.635&	0.589\\
&720 &0.142 &0.299 &0.127 &0.280 &\textbf{0.126}&\textbf{0.283}&	0.183&	0.355&	0.475&	0.628&	0.762&	0.666\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
&96 &\textbf{0.128} &\textbf{0.271} &0.156 &0.306 & 0.153&	0.306&	0.213&	0.373&	0.217&	0.379&	1.411&	0.838\\
&192 &\textbf{0.185} &\textbf{0.330} &0.238 &0.380 & 0.204&	0.351&	0.227&	0.387&	0.281&	0.429&	5.658&	1.671\\
&336 &\textbf{0.231} &\textbf{0.378} &0.271 &0.412 & 0.246&	0.389&	0.242&	0.401&	0.293&	0.437&	4.777&	1.582\\
&720 &0.278 &0.420 &0.288 &0.438 & \textbf{0.268}&	\textbf{0.409}&	0.291&	0.439&	0.218&	0.387&	2.042&	1.039\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
&96 &\textbf{0.033} &\textbf{0.140} &0.036 &0.149 & 0.056&	0.183&	0.109&	0.277&	0.049&	0.171&	0.296&	0.355\\
&192 &\textbf{0.058} &\textbf{0.186} &0.069 &0.206 & 0.081&	0.216&	0.151&	0.310&	0.157&	0.317&	0.429&	0.474\\
&336 &0.084 &0.231 &\textbf{0.071} &\textbf{0.209} & 0.076&	0.218&	0.427&	0.591&	0.289&	0.459&	0.585&	0.583\\
&720 &\textbf{0.102} &0.250 &0.105 &\textbf{0.248} & 0.110&	0.267&	0.438&	0.586&	0.430&	0.579&	0.782&	0.730\\
\midrule
\multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
& 96 & 0.067 & 0.198 &\textbf{0.063} &\textbf{0.189} & 0.065 & 0.189 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
& 192 & \textbf{0.102} & \textbf{0.245} &0.110 &0.252 & 0.118 & 0.256 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
& 336 & \textbf{0.130} & \textbf{0.279} &0.147 &0.301 & 0.154 & 0.305  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
& 720 & \textbf{0.178} & \textbf{0.325} &0.219 &0.368 & 0.182 &0.335  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
\bottomrule
\end{tabular}
}
\label{tab:uni-benchmarks-ett}
% \end{adjustwidth}
% \end{small}
\end{table*}

% \begin{table*}[t]
% \centering
% % \begin{small}
% % \begin{adjustwidth}{-1.5in}{-1in}
% \caption{Univariate long sequence time-series forecasting results on ETT full benchmark. The best results are highlighted in bold.}
% \vskip 0.05in
% \scalebox{0.85}{
% \begin{tabular}{c|c|cccccccccccccccc}
% \toprule
% \multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FEDformer-f}&\multicolumn{2}{c|}{FEDformer-w}&\multicolumn{2}{c|}{Autoformer}&\multicolumn{2}{c|}{Informer}&\multicolumn{2}{c|}{LogTrans}&\multicolumn{2}{c}{Reformer}\\
% \midrule
% \multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
% \midrule

% \multirow{4}{*}{\rotatebox{90}{$ETTh1$}}
% &96 &0.079 &0.215 &0.080 &0.214 &\textbf{0.071} &\textbf{0.206}&	0.193&	0.377&	0.283&	0.468&	0.532&	0.569\\
% &192 &\textbf{0.104} &\textbf{0.245} &0.105 &0.256 & 0.114&	0.262&	0.217&	0.395&	0.234&	0.409&	0.568&	0.575\\
% &336 &0.119 &0.270 &0.120 &0.269 &\textbf{0.107}&\textbf{0.258}&	0.202&	0.381&	0.386&	0.546&	0.635&	0.589\\
% &720 &0.142 &0.299 &0.127 &0.280 &\textbf{0.126}&\textbf{0.283}&	0.183&	0.355&	0.475&	0.628&	0.762&	0.666\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTh2$}}
% &96 &\textbf{0.128} &\textbf{0.271} &0.156 &0.306 & 0.153&	0.306&	0.213&	0.373&	0.217&	0.379&	1.411&	0.838\\
% &192 &\textbf{0.185} &\textbf{0.330} &0.238 &0.380 & 0.204&	0.351&	0.227&	0.387&	0.281&	0.429&	5.658&	1.671\\
% &336 &\textbf{0.231} &\textbf{0.378} &0.271 &0.412 & 0.246&	0.389&	0.242&	0.401&	0.293&	0.437&	4.777&	1.582\\
% &720 &0.278 &0.420 &0.288 &0.438 & \textbf{0.268}&	\textbf{0.409}&	0.291&	0.439&	0.218&	0.387&	2.042&	1.039\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm1$}}
% &96 &\textbf{0.033} &\textbf{0.140} &0.036 &0.149 & 0.056&	0.183&	0.109&	0.277&	0.049&	0.171&	0.296&	0.355\\
% &192 &\textbf{0.058} &\textbf{0.186} &0.069 &0.206 & 0.081&	0.216&	0.151&	0.310&	0.157&	0.317&	0.429&	0.474\\
% &336 &0.084 &0.231 &\textbf{0.071} &\textbf{0.209} & 0.076&	0.218&	0.427&	0.591&	0.289&	0.459&	0.585&	0.583\\
% &720 &\textbf{0.102} &0.250 &0.105 &\textbf{0.248} & 0.110&	0.267&	0.438&	0.586&	0.430&	0.579&	0.782&	0.730\\
% \midrule
% \multirow{4}{*}{\rotatebox{90}{$ETTm2$}} 
% & 96 & 0.067 & 0.198 &\textbf{0.063} &\textbf{0.189} & 0.065 & 0.189 & 0.088 & 0.225 & 0.075 & 0.208 & 0.076  &0.214   \\
% & 192 & \textbf{0.102} & \textbf{0.245} &0.110 &0.252 & 0.118 & 0.256 & 0.132 &0.283 & 0.129 &0.275  & 0.132  & 0.290   \\
% & 336 & \textbf{0.130} & \textbf{0.279} &0.147 &0.301 & 0.154 & 0.305  &0.180 &0.336 & 0.154 &0.302  & 0.160  & 0.312    \\
% & 720 & \textbf{0.178} & \textbf{0.325} &0.219 &0.368 & 0.182 &0.335  &0.300  &0.435 & 0.160 &0.321  & 0.168  &0.335     \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:uni-benchmarks-ett}
% % \end{adjustwidth}
% % \end{small}
% \end{table*}

==> tables_new/4.2b_M4_benchmark.tex <==
%\resizebox{!}{\.5\paperheight}{
% \vskip -0.2in
\begin{table*}[h]
\centering
%\begin{footnotesize}
% \begin{adjustwidth}{-1.5in}{-1in}
\caption{Multivariate long-term series forecasting results on six datasets with various input length and prediction length $O \in \{96,192,336,720\}$ (For ILI dataset, we set prediction length $O \in \{24,36,48,60\}$). A lower MSE indicates better performance. All experiments are repeated 5 times.}\vspace{-1mm}
\scalebox{0.80}{
\begin{tabular}{c|c|cccccccccccccccccc}
\toprule
\multicolumn{2}{c|}{Methods}&\multicolumn{2}{c|}{FiLM+xxx}&\multicolumn{2}{c|}{FEL+xxx}&\multicolumn{2}{c|}{Gconv+xxx}&\multicolumn{2}{c|}{S4}\\
\midrule
\multicolumn{2}{c|}{Metric} & MSE  & MAE & MSE & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE& MSE  & MAE\\
\midrule
\multirow{4}{*}{\rotatebox{90}{ETTm2}} &96 & \textbf{0.165} & \textbf{0.256} &0.203 &0.287 &0.255  &0.339 &0.705 &0.690 &0.365  &0.453  &0.768  &0.642  &0.658  &0.619    \\
                        & 192 & \textbf{0.222} & \textbf{0.296} &0.269  &0.328  &0.281 &0.340 &0.924 &0.692 &0.533  &0.563  &0.989  &0.757  &1.078  &0.827    \\
                        & 336 & \textbf{0.277} & \textbf{0.333} & 0.325 &0.366 &0.339  &0.372 &1.364 &0.877 &1.363&0.887  &1.334  &0.872  &1.549  &0.972     \\
                        & 720 & \textbf{0.371} & \textbf{0.389} &0.421 &0.415 &0.422  &0.419 &0.877 &1.074 &3.379  &1.338 & 3.048 &1.328  &2.631  &1.242      \\
\midrule
\multirow{4}{*}{\rotatebox{90}{Electricity}} &96  &\textbf{0.154}  &\textbf{0.267}  &0.183 &0.297 &0.201  &0.317 &0.304 &0.405 &0.274  &0.368  &0.258  &0.357  &0.312  &0.402    \\
                        & 192 &\textbf{0.164} & \textbf{0.258} & 0.195 &0.308 &0.222  &0.334 &0.313 &0.413 &0.296 &0.386  &0.266 &0.368  &0.348  &0.433    \\
                        & 336 & \textbf{0.188} & \textbf{0.283} &0.212 &0.313 &0.231 &0.338 &0.290 &0.381 &0.300  &0.394  &0.280 &0.380  &0.350  & 0.433    \\
                        & 720 & 0.236 & \textbf{0.332} &\textbf{0.231} &0.343 &0.254  &0.361 &0.262 &0.344 &0.373  &0.439 &0.283  &0.376  &0.340  &0.420     \\

\bottomrule
\end{tabular}
\label{tab:multi-benchmarks}
}
% \end{adjustwidth}
%\end{footnotesize}
\end{table*}
%}
